Approximation Rate of the Transformer Architecture for Sequence Modeling

The Transformer architecture is widely applied in sequence modeling applications, yet the theoretical understanding of its working principles remains limited. In this work, we investigate the approximation rate for single-layer Transformers with one head. We consider a class of non-linear relationships and identify a novel notion of complexity measures to establish an explicit Jackson-type approximation rate estimate for the Transformer. This rate reveals the structural properties of the Transformer and suggests the types of sequential relationships it is best suited for approximating. In particular, the results on approximation rates enable us to concretely analyze the differences between the Transformer and classical sequence modeling methods, such as recurrent neural networks.

==> 6.compare_backup.tex <==
\section{Comparison with RNN}\label{sec: 6 compare}
Based on the approximation results in \cref{thm: approximation rate}, 
this section presents a comparison between the Transformer and RNN.
Our comparison focuses on the handling of the change in the temporal structures of the target.
We primarily focus on two distinct temporal structures: 
temporal ordering and temporal mixing,
which have different effects on the complexity measures of each architecture.
We will manipulate the temporal structures of input sequences while keeping the output unchanged. 
This manipulation will lead to alterations in the underlying temporal structures of the sequential relationships, allowing us to assess how each architecture responds to such changes.

\paragraph{Temporal Ordering Structure}
We first analyze how the ordering of the input sequences affects the sequential relationships. 
Empirically, 
it is observed that in certain contexts, 
the ordering of inputs does not significantly impact the relationships. 
For instance, in NLP applications, 
altering the word order in a sentence often does not drastically change its meaning. 
Similarly, in the ViT model, 
the arrangement of image patches typically does not substantially affect the outcome. 
However, 
in specific applications such as time series analysis, 
temporal ordering plays a crucial role, 
as the target relationships are predominantly governed by the ordering of the sequence.

We examine a linear relationship defined by the equation
$
y(t) = \sum_{s=0}^t \rho(s) x(t-s).
$
This relationship is determined by the kernel function $\rho(s)$. 
Consider $\rho_1(s)=\exp{(-s)}$ as an instance where temporal ordering is significant. 
In this scenario, 
any alteration in the input sequence directly affects the kernel function $\rho$ itself, 
underlining the importance of temporal ordering.
On the other hand, 
for a kernel function like $\rho_2(s)$, 
composed of random numbers, 
temporal ordering loses its significance. 
This is because any change in the sequence of inputs results in a different, 
but still randomly generated $\rho_2$. 
This example illustrates how the relevance of temporal ordering can vary depending on the nature of the kernel function.

We also take into account permuted targets,
where we apply the same temporal permutation to the entire input dataset while keeping the output unchanged. 
For the linear target relation, 
this is equivalent to permuting the kernel function $\rho$.
This allows us to evaluate how sensitive the model is to changes in the temporal ordering of the input data.
We next utilize both RNN and the Transformer to learn these targets. 
The results are shown in \cref{tab: tab1}.
\begin{table}[htbp] 
    \centering
    % \small % or \footnotesize
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}{*}{} & \multicolumn{2}{c}{With TO} & \multicolumn{2}{c}{Without TO} \\
    \cline{2-5}
                      & \multicolumn{1}{c}{RNN} & Trans. & \multicolumn{1}{c}{RNN} & Trans. \\ \midrule
    Original          & \multicolumn{1}{c}{$1.02e{-7}$}   &  $2.18e{-5}$          & \multicolumn{1}{c}{$5.58$}   & $5.43e{-4}$           \\
    Permuted          & \multicolumn{1}{c}{$3.57e{-2}$}   & $2.51e{-5}$           & \multicolumn{1}{c}{$5.24$}   & $5.36e{-4}$         \\ \bottomrule
    \end{tabular}
    \caption{The table presents the MSE values for both RNN and the Transformer on different dataset settings. 
    In the permuted setting, all input sequences are permuted using a fixed permutation, 
    resulting in a change in the underlying temporal ordering (TO).}
    \label{tab: tab1}
\end{table}
We first observe that in datasets with temporal ordering dependency, 
RNNs tend to achieve better performance.
Moreover, 
when the input sequences are permuted, 
thereby altering the temporal order, 
the performance of RNNs noticeably decreases, 
while the Transformer remains unaffected by such permutations.
On the other hand, in datasets with minimal temporal dependencies, 
the Transformer exhibits better performance. 
Additionally, when the input sequences are permuted in datasets without temporal ordering, 
the performance impact is relatively minor since there is no underlying temporal ordering to disrupt.

These phenomena can indeed be deduced from the Jackson-type results. 
Let's first look at the RNNs.
According to Jackson-type rates for RNNs as presented in \citet{li2022.ApproximationOptimizationTheory}, 
the complexity measure of the target is determined by the decay and smoothness of $\rho$. 
Consequently, for RNNs, the temporal ordering becomes important. 
Changing the temporal order of $\rho_1(s)$ may break its decaying pattern as well as its smoothness,
which will increase its complexity measure within the RNN hypothesis space.
This explains the performance drop of RNN when we alter the temporal ordering of the targets.
However, 
\cref{thm: approximation rate} suggests that the Transformer is unaffected by temporal ordering. 
This is because all of its complexity measures only consider pointwise functions. 


\paragraph{Impact of Temporal Ordering on the Transformer}
We consider a fixed permutation denoted as $p$, 
and the associated permuted target relationship given by ${H}\depen{p}_t(\bm x) = H_t(\bm x \circ p)$, 
where all input sequences have their temporal indices permuted by the common permutation $p$. 
By applying this permutation, 
the temporal ordering of the target is completely altered.
The Transformer (with positional encoding) can learn both relationships in the same manner without the need for additional parameters. 
Specifically, if we have a piecewise function $\hat f$ on $\I_1 \cdots \I\tau$ such that $\hat f(x_s)=\hat f_s(x_s)$ for $x_s\in\I_s$, 
we can construct another feed-forward network $\hat g$ in such a way that $\hat g(x_{p(s)}) = \hat f_s(x_s)$. 
Here, $\hat g$ represents a permutation of the function domain of each piece.
By changing $\hat g$ into $\hat f$,
we achieve a modified model that learns the permuted target relationships.
This implies that temporal ordering does not affect the performance of the Transformer.
This point is further substantiated by our testing of the Transformer on real-world datasets,
as illustrated in \cref{tab: tab2}. 
Specifically, 
we consider the ViT model on the CIFAR10 dataset and the base Transformer structure \cite{vaswani2017.AttentionAllYou} on the WMT2014 English-German dataset. 
In the case of the permuted dataset, 
we fix a permutation of indices denoted as $p$ and apply it to all inputs while keeping the output unchanged. 
These experimental results provide strong evidence that the performance of the Transformer is predominantly unaffected by temporal ordering.

Some variants of the Transformer, 
such as Informer \cite{zhou2021.InformerEfficientTransformer} and Autoformer \cite{wu2022.AutoformerDecompositionTransformers}, 
have been proposed specifically to address temporal relationships, 
particularly in sequence forecasting tasks. 
However, 
empirical results presented in \citet{zeng2022.AreTransformersEffective} indicate that these variants still cannot effectively capture temporal relationships. 



\begin{table}[htbp] 
    \centering
    % \small % or \footnotesize
    \begin{tabular}{ccc}
    \toprule
    & CIFAR10 (\textit{Acc.}) & ENG-DE (\textit{BLUE}) \\
    \cline{1-3}
    Original          & \multicolumn{1}{c}{$0.98$}   &  $26.85$                   \\
    Permuted          & \multicolumn{1}{c}{$0.96$}   & $25.91$                   \\ \bottomrule
    \end{tabular}
    \caption{The experiment results of the Transformer on original and permuted datasets.}
    \label{tab: tab2}
\end{table}


In summary, 
The inability to capture temporal order can be seen as both an advantage and a disadvantage for
the Transformer. 
On the one hand, RNNs can outperform the Transformer in modeling relationships with
strong temporal order dependencies. However, the Transformer excels in tasks that involve little temporal
dependencies.



\section{Conclusion}

In this paper, 
we have developed Jackson-type approximation rates for the Transformer in a simplified setting. 
An important outcome of our work is the identification of complexity measures that define the approximation space defined in \cref{eq: approximation space}. 
This, in turn, 
enables us to derive explicit Jackson-type approximation rate results in \cref{thm: approximation rate}. 
Our rate results suggest that the Transformer performs well when the target exhibits a low-rank pattern.
The experiments presented in \cref{sec: 5 experiments} showcase the existence of low-rank patterns in real-world applications.
Furthermore, 
the comparisons with RNNs underscore the specific temporal structures that each model is proficient at handling.
Future research directions may involve extending the analysis to multi-headed attention and deeper Transformers.
